How I Learned to Stop Worrying About User-Visible Endpoints and Love MPI

MPI+threads is gaining prominence as an alternative to the traditional MPI everywhere model in order to better handle the disproportionate increase in the number of cores compared with other on-node resources. However, the communication performance of MPI+threads can be 100x slower than that of MPI everywhere. Both MPI users and developers are to blame for this slowdown. Typically, MPI users do not expose logical communication parallelism. Consequently, MPI libraries use conservative approaches, such as a global critical section, to maintain MPI's ordering constraints for MPI+threads, thus serializing access to parallel network resources and hurting performance. To enhance MP+threads' communication performance, researchers have proposed MPI Endpoints as a user-visible extension to MPI-3.1. MPI Endpoints allows a single process to create multiple MPI ranks within a communicator. This could allow each thread to have a dedicated communication path to the network and improve performance. The onus of mapping threads to endpoints, however, would then be on domain scientists. We play the role of devil's advocate and question the need for user-visible endpoints. We certainly agree that dedicated communication channels are critical. To what extent, however, can we hide these channels inside the MPI library without modifying the MPI standard and thus unburden the user? More important, what functionality would we lose through such abstraction? This paper answers these questions through a new MPI-3.1 implementation that uses virtual communication interfaces (VCIs). VCIs abstract underlying network contexts. When users expose parallelism through existing MPI mechanisms, the MPI library maps that parallelism to the VCIs, relieving domain scientists from endpoints. We identify cases where VCIs perform as well as user-visible endpoints, as well as cases where such abstraction hurts performance.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=main

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf: $(PACKAGE).tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<


%.cls:   %.ins %.dtx
	pdflatex $<




.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut main.pdf

distclean: clean

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst

